Bridging the Safety Gap: A Guardrail Pipeline for Trustworthy LLM Inferences

We present Wildflare GuardRail, a guardrail pipeline designed to enhance the safety and reliability of Large Language Model (LLM) inferences by systematically addressing risks across the entire processing workflow. Wildflare GuardRail integrates several core functional modules, including Safety Detector that identifies unsafe inputs and detects hallucinations in model outputs while generating root-cause explanations, Grounding that contextualizes user queries with information retrieved from vector databases, Customizer that adjusts outputs in real time using lightweight, rule-based wrappers, and Repairer that corrects erroneous LLM outputs using hallucination explanations provided by Safety Detector. Results show that our unsafe content detection model in Safety Detector achieves comparable performance with OpenAI API, though trained on a small dataset constructed with several public datasets. Meanwhile, the lightweight wrappers can address malicious URLs in model outputs in 1.06s per query with 100% accuracy without costly model calls. Moreover, the hallucination fixing model demonstrates effectiveness in reducing hallucinations with an accuracy of 80.7%.

==> tables_and_algos/safety_detection_exp.tex <==

\begin{table}[ht]
\centering
\caption{Unsafe Content Detection Comparison}
\label{tab:toxicity detecion}
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Model} & \textbf{Accuracy} & \textbf{Recall} & \textbf{F1} \\ \midrule
Detoxify-Roberta~\cite{Detoxify} & 0.847 & 0.504 & 0.483 \\
Detoxify-BERT~\cite{Detoxify} & 0.872 & 0.568 & 0.585 \\
NeMo & 0.687 & 0.767 & 0.611 \\
OpenAI Moderate~\cite{openai-data-paper} & 0.878 & 0.573 & 0.595 \\
PerspectiveAPI~\cite{perspective-api} & 0.875 & 0.573 & 0.594 \\
Ours & 0.877 & 0.624 & 0.656 \\
\bottomrule
\end{tabular}
\end{table}

==> tables_and_algos/safety_detector_training_data_table.tex <==

\begin{table}[ht]
\centering
\small
\caption{Training data for unsafe content detection}
\label{tab: input_detection_training_data}
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Dataset} & \textbf{Train} & \textbf{Validation} & \textbf{Test} \\ \midrule
HEx-PHI~\citep{anonymous2024finetuning} & 330 & 0 & 0 \\
OpenAI~\citep{openai-data-paper}& 160 & 1,500 & 0 \\
Hotpot QA~\citep{yang2018hotpotqa} & 3,000 & 2,500 & 500 \\
Truthful QA~\citep{lin2021truthfulqa} & 500 & 100 & 100 \\
Awesome ChatGPT Prompts~\citep{awesome-chatgpt-prompts} & 0 & 150 & 0 \\
Jigsaw Unintended-Bias Data~\citep{jigsaw-unintended-bias-in-toxicity-classification} & 100,000 & 2,000 & 300 \\
GPT-Jailbreak~\citep{ChatGPT-Jailbreak-Prompts} & 0 & 78 & 0 \\
Jailbreak~\cite{jailbreak-classification} & 400 & 0 & 70 \\
Personalization Prompt~\citep{filtered_personalization_prompt_response} & 1,000 & 800 & 200 \\
QA Chat Prompts~\citep{qa-chat-prompts} & 0 & 200 & 0 \\
ChatGPT Prompts~\citep{ChatGPT-prompts} & 350 & 0 & 0 \\
10k Prompts Ranked~\citep{10k_prompts_ranked} & 500 & 500 & 200 \\
Iterative Prompt~\citep{iterative-prompt-v1-iter1-20K} & 500 & 500 & 200 \\
Instruction Following~\citep{instruction-following} & 200 & 340 & 0 \\
\bottomrule
\end{tabular}
\label{tb: unsafe_content_detection_datasets}
\end{table}

==> tables_and_algos/top-k_callbacks_table.tex <==

\begin{table}[htbp]
\centering
\caption{Callbacks of Original Data Records in Top-$k$ Queries}
\label{tab:exp-query-call-back}
\small
\begin{tabular}{@{}llcccccccc@{}}
\toprule
\textbf{Dataset} & \textbf{Query Type} & \multicolumn{4}{c}{\textbf{Whole Knowledge Indexing}} & \multicolumn{4}{c}{\textbf{Key Information Indexing}} \\ 
\cmidrule(lr){3-6} \cmidrule(l){7-10}
& & \textbf{Top1} & \textbf{Top3} & \textbf{Top5} & \textbf{Top10} & \textbf{Top1} & \textbf{Top3} & \textbf{Top5} & \textbf{Top10} \\
\midrule
\multirow{2}{*}{E-Commerce} & Original & 0.96 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
                                                      & Rephrased & 0.82 & 1.00 & 1.00 & 1.00 & 0.92 & 0.98 & 1.00 & 1.00 \\
\addlinespace
\multirow{2}{*}{ChatDoctor}                  & Original & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
                                                      & Rephrased & 0.66 & 0.78 & 0.80 & 0.82 & 0.88 & 0.94 & 0.96 & 0.98 \\
\addlinespace
\multirow{2}{*}{PatientDoctorChat}          & Original & 0.72 & 0.90 & 0.96 & 0.98 & 0.96 & 1.00 & 1.00 & 1.00 \\
                                                      & Rephrased & 0.56 & 0.74 & 0.76 & 0.80 & 0.78 & 0.92 & 0.94 & 0.96 \\
\bottomrule
\end{tabular}
\end{table}
